Constant Query Local Decoding Against Deletions Is Impossible

Locally decodable codes (LDC's) are error-correcting codes that allow recovery of individual message indices by accessing only a constant number of codeword indices. For substitution errors, it is evident that LDC's exist -- Hadamard codes are examples of $2$-query LDC's. Research on this front has focused on finding the optimal encoding length for LDC's, for which there is a nearly exponential gap between the best lower bounds and constructions. Ostrovsky and Paskin-Cherniavsky (ICITS 2015) introduced the notion of local decoding to the insertion and deletion setting. In this context, it is not clear whether constant query LDC's exist at all. Indeed, in contrast to the classical setting, Block et al. conjecture that they do not exist. Blocki et al. (FOCS 2021) make progress towards this conjecture, proving that any potential code must have at least exponential encoding length. Our work definitively resolves the conjecture and shows that constant query LDC's do not exist in the insertion/deletion (or even deletion-only) setting. Using a reduction shown by Blocki et al., this also implies that constant query locally correctable codes do not exist in this setting.

==> 2query.tex <==
\section{Impossibility of $2$-Query Deletion LDC's} \label{sec:2query}

In this section, we show the following theorem.

\begin{theorem}\label{thm:2query}
    For any $\eps>0$, there exists a constant $C(\eps)$ such that for all $n>C(\eps)$, there is no $2$-query $\eps$-resilient LDC.
\end{theorem}

We'll show this theorem by considering any LDC $\C$ and describing a corruption pattern for which some index $i$ cannot be recovered with only $2$ queries. Throughout this section, $\eps$ and $n$ are fixed, $\C$ denotes the candidate LDC (encoding strings of length $n$ to length $M=2^m$), $x$ denotes a message being sent (which the adversary is oblivious to), and $z$ typically is an arbitrary string of length $M$.

We remark that the assumption that $M$ is a power of $2$ is without loss of generality. This is because any encoding is effectively padded with infinitely many $0$'s since out-of-bounds queries return $0$. To make the code's length a power of $2$, simply increase the length of the code until the next power of $2$ larger than $M$ which at most doubles the total length. Then, any adversarial attack on the new padded encoding also works on the original (since deleting indices larger than $M$ doesn't change the string) and requires (at most) the same number of deletions, but since $M$ at most doubled in length, this only doubles the value of $\eps$. 

\subsection{Definitions and Useful Lemmas}

We begin with a few useful definitions and simple facts.

\begin{definition}[$\W{t}{b}{z}$ and $\W{t}{b}{z}$] \label{def:W}
    We define the layer $t$ weight $\W{t}{b}{z}$ of a string $z \in \{0,1\}^{2^m}$ as follows. For any chunk $C$, let $v_0(C)$ denote the fraction of the chunk that is $0$'s and $v_1(C)$ denote the fraction of the chunk that is $1$'s. Then for $b\in \{0,1\}$, let 
    \[
        \W{t}{b}{z}:= \mathop{\bbE}_{i\in [2^{m-t}]} \Big[ v_b(C_t(z)[i])^2 \Big].
    \]

    We define the cumulative weight of the code $\C : \{0,1\}^n \to \{0,1\}^M$ as follows:
    \[
        \W{t}{b}{\C}:= \mathop{\bbE}_{x\in \{0,1\}^n} \left[ \W{t}{b}{\C(x)} \right].
    \]
    For convenience of notation, for $t>m$, we let $\W{t}{b}{x}:=-1$ and so $\W{t}{b}{\C}=-1$. Similarly for $t\leq 0$, we let $\W{t}{b}{x}:=2$ and so $\W{t}{b}{\C}=2$. This will be useful to create a gap between $\W{t}{b}{x}$ and $\W{m}{b}{x}$ for $t>m$ (and a similar gap when $t<0$).
\end{definition}

\begin{lemma}
    For a given string $b\in \{0,1\}$ and $z\in\{0,1\}^M$, the function $\W{t}{b}{z}$ is monotonically decreasing with $t$. Consequently, $\W{t}{b}{\C}$ is monotonically decreasing with $t$.
\end{lemma}

\begin{proof}
    We will demonstrate for any $1\leq t < m$ that $\W{t+1}{b}{z}\leq \W{t}{b}{z}$. Recall that by definition, $\W{t}{b}{z} = \bbE_{i\in [2^{m-t}]}v_b(C_t(z)[i])^2$. Then, we have
    \begin{align*}
        \W{t+1}{b}{z} &= \mathop{\bbE}_{i\in [2^{m-t-1}]} \Big[ v_b(C_{t+1}(z)[i])^2 \Big] \\
        &= \mathop{\bbE}_{i\in [2^{m-t-1}]} \left[ \left(\frac{v_b(C_t(z)[2i-1]) + v_b(C_t(z)[2i])}{2}\right)^2 \right] \\
        &\leq \mathop{\bbE}_{i\in [2^{m-t-1}]} \left[ \frac{v_b(C_t(z)[2i-1])^2 + v_b(C_t(z)[2i])^2}{2} \right] \\
        &= \mathop{\bbE}_{i\in [2^{m-t}]} \Big[ v_b(C_t(z)[i])^2 \Big] \\
        &= \W{t}{b}{z}
    \end{align*}
    as desired. It follows that $\W{t}{b}{\C}$ is monotonically decreasing as well.
\end{proof}

\begin{definition} [Critical Layer]
    Given $0<\delta<1$ where $\frac1\delta$ is an integer, we say that a layer $t \in [m]$ is $\delta$-\emph{critical} for $\C$ if for some $k\in \bbZ$, it holds that $\W{t}{b}{\C} < k\delta \leq \W{t+1}{b}{\C}$. In other words, there is one critical layer every time the value of $\W{t}{b}{\C}$ viewed as a function of $t$ changes by about $\delta$.
\end{definition}

\begin{lemma} \label{lem:const-crit-layers}
    For any $\delta>0$, there are at most $\delta^{-10}$ layers that are $\delta$-critical for $\C$.
\end{lemma}

\begin{proof}
    trivial combo
\end{proof}

\begin{lemma}
    If for some $1\leq a < c \leq m$, none of the layers $t$ with $a \leq t < c$ are $\delta^3$-critical for $\C$, then for at most $\delta$-fraction of the values of $x\in \{0,1\}^n$, it holds that $\W{t-\frac1\delta}{b}{\C(x)} - \W{t+\frac1\delta}{b}{\C(x)} > \frac1\delta$ where $b\in \{0,1\}$.
\end{lemma}

\begin{proof}
    Because none of the layers between $a$ and $c$ are $\delta^2$-critical, it must hold that $\W{a}{b}{\C} - \W{c}{b}{\C}\leq 2\delta^2$. Otherwise it is guaranteed that some multiple of $\delta^2$ would fall within the range. Moreover, let us assume for the sake of contradiction that for more than $\delta$-fraction of the values of $x$, that $\W{t-\frac1\delta}{b}{\C(x)} - \W{t+\frac1\delta}{b}{\C(x)} > \frac1\delta$.
    
    Then, we can see that
    \[
        2\delta^3 \geq \W{t-\frac1\delta}{b}{\C} - \W{t+\frac1\delta}{b}{\C} = \mathop{\bbE} \left[ \W{t-\frac1\delta}{b}{z} - \W{t+\frac1\delta}{b}{z} \right] \geq \delta\cdot \delta + (1-\delta)\cdot 0 = \delta^2
    \]
    which is a contradiction as long as $\delta<\frac12$.
\end{proof}

Finally, we define the adversary's randomized corruption process for performing deletions. We remind the reader that the adversary chooses what to delete depending on the code $\C$ but not the individual choice of $x$ or $\C(x)$. The decoder knows the randomized algorithm used to perform the deletions, but obviously not the specific choice of randomness.

\paragraph{Adversary's corruption process.} We describe how the adversary corrupts a string $z$ of length $M$. Recall that each layer $t$, the string $z$ is partitioned into chunks of length $2^t$ denoted $C_t(z)$. We modify every layer $t$ that is $\eps^{10}$-critical or within $\eps^{-10}$ of a critical layer and call such layers \emph{modified layers}. The modification (deletion) process is as follows. For each chunk $1\leq i \leq 2^{m-t}$, choose $\eps_{t,i}$ uniformly at random in the interval $[0,\eps^{200}]$. Then, for the layers $t$ in order, starting with the layer corresponding to the smallest value of $t$, delete the first $\left\lfloor \eps_{t,i}\cdot 2^t \right\rfloor$ remaining bits in the chunk. 

Note that there will always be at least these many bits remaining to delete; for any chunk $C_t(z)$, each modified layer before $t$ deleted at most $\eps^{200}$-fraction of the bits in $C_t(z)$. There are at most $\eps^{-100}$ critical layers (Lemma~\ref{lem:const-crit-layers}), so at most $2\eps^{-110}$ modified layers, so at most $2\eps^{-90}$ of the chunk had been deleted. Moreover, this argument makes clear that at most $\eps$ fraction of the code was deleted overall.

\begin{remark}
We remark (explained in detail in Section~\ref{sec:overview}) that a simpler corruption process is likely possible to analyze with a similar proof method in the case of two queries; however, the one presented here better mirrors the analysis of the $k$-query case. The alternative deletion pattern (that we do not use) is as follows: choose $\eps_1\in [\eps/4,\eps/2]$ and $\eps_2\in [\eps^2/4,\eps^2/2]$, and delete the first $\eps_1$ bits and then every remaining $1/\eps_2$'th bit. This is very similar to the corruption process used by~\cite{BlockiCGLZZ21} in showing the exponential lower bound on $2$-query deletion LDC's.
\end{remark}

\subsection{Analysis of Distribution of Query Outputs}

In this section, we introduce the central lemma used in the proof of Theorem~\ref{thm:2query}. We begin with a high-level overview of the proof.

Recall that the decoder conducts two queries, denoted as $\widehat{q_1}$ and $\widehat{q_2}$, to the corrupted string. For each query pair, the resulting output corresponds to a specific distribution on $\{0,1\}^2$ depending on Alice's message $x$. In this sense, the query pair can be treated as a function mapping from ${0,1}^N$ (representing Alice's message $x$) to $\cD({0,1}^2)$ (representing the resultant distribution). There are many pairs of queries Alice can make; in fact $\approx N^2$ such pairs. The main idea of the proof is to demonstrate that there are a \emph{constant} number of functions $\cF_1,\ldots , \cF_{K(\eps)} : \{0,1\}^N \to \cD(\{0,1\}^2)$ such that every query pair corresponds approximately to some $\cF_i$. That is, executing queries $\widehat{q_1},\widehat{q_2}$ when Alice has message $x$ is akin to drawing from the distribution $\cF_(x)$. From here, we conclude in Section~\ref{sec:2query-info} using an info-theoretic argument that $N$ cannot be much larger than $K(\eps)$.

Formally, the lemma we want to prove is as follows.

\begin{restatable}{lemma}{constfns} \label{lem:const-fns}
    There is a constant $K(\eps)$ so that there are functions $\cF_1,\ldots , \cF_{K(\eps)} : \{0,1\}^N \to \cD(\{0,1\}^2)$ so that for any two queries $\widehat{q_1},\widehat{q_2}$, there is some $i \in [K(\eps)]$ such that 
    \[
        \BigV \cF_i, \C(x)[\cD(\widehat{q_1},\widehat{q_2})] \BigV_\TV \leq \eps^2.
    \]
\end{restatable}

We split the proof of this lemma into two parts. In the first lemma, we show that for any pair of queries where $t=\lfloor \log(\widehat{q_2}-\widehat{q_1}) \rfloor-1$ corresponds to a modified layer (of which there are only constantly many), for each value of $t$ there are only a constant number of functions needed to approximate any pair of queries.

\begin{lemma} \label{lem:mod-layers}
    There is a constant $\alpha(\eps)$ so that for any modified layer $t\in [m]$, the following holds. There are functions $\varphi^{(t)}_1,\ldots , \varphi^{(t)}_{\alpha(\eps)} : \{0,1\}^N \to \cD(\{0,1\}^2)$ so that for any two queries $\widehat{q_1},\widehat{q_2}$ with $t=\lfloor \log(\widehat{q_2}-\widehat{q_1}) \rfloor-1$, there is some $i \in [\alpha(\eps)]$ such that 
    \[
        \BigV \varphi^{(t)}_i, \C(x)[\cD(\widehat{q_1},\widehat{q_2})] \BigV_\TV \leq \eps^2.
    \]
\end{lemma}

The second lemma deals with the case where $t=\lfloor \log(\widehat{q_2}-\widehat{q_1}) \rfloor-1$ is not a modified layer. In this case, we show that there is constant-sized set of functions independent of $t$ that approximate any pair of queries. Since the number of non-modified layers is super-constant, the set of functions needs to be the same for all values of $t$ (so there are only a constant number of functions used overall).

\begin{lemma} \label{lem:nonmod-layers}
    There is a constant $\beta(\eps)$ so that the following holds. There are functions $\varphi_1,\ldots , \varphi_{\beta(\eps)} : \{0,1\}^N \to \cD(\{0,1\}^2)$ so that for any two queries $\widehat{q_1},\widehat{q_2}$ where $t=\lfloor \log(\widehat{q_2}-\widehat{q_1}) \rfloor-1$ is not a modified layer, there is some $i \in [\beta(\eps)]$ such that 
    \[
        \BigV \varphi_i, \C(x)[\cD(\widehat{q_1},\widehat{q_2})] \BigV_\TV \leq \eps^2.
    \]
\end{lemma}

Next, we show formally how Lemma~\ref{lem:const-fns} follows from Lemma~\ref{lem:mod-layers} and Lemma~\ref{lem:nonmod-layers}.

\begin{proof}[Proof of Lemma~\ref{lem:const-fns}]
    We let the functions $\cF_i$ be the union of $\varphi_1,\ldots , \varphi_{\beta(\eps)}$ from Lemma~\ref{lem:nonmod-layers} and $\varphi^{(t)}_1,\ldots , \varphi^{(t)}_{\alpha(\eps)}$ from Lemma~\ref{lem:mod-layers}. It is clear that any pair of queries $\widehat{q_1},\widehat{q_2}$ is approximated by one of these functions; if the layer $t=\lfloor \log(\widehat{q_2}-\widehat{q_1}) \rfloor-1$ is modified, then we use the functions from Lemma~\ref{lem:mod-layers} and otherwise the functions from Lemma~\ref{lem:nonmod-layers}
    
    In order to prove that this set is constant-sized, we need to show that there are only a constant number of modified layers. By Lemma~\ref{lem:const-crit-layers}, there are at most $\eps^{-100}$ critical layers, and each yields at most $2\eps^{-10}$ modified layers, for a total of $2\eps^{-110}$ modified layers.
\end{proof}

Finally, in the next two subsections, we prove Lemma~\ref{lem:mod-layers} and Lemma~\ref{lem:nonmod-layers}.

\subsubsection{Proof of Lemma~\ref{lem:mod-layers}}

% \begin{lemma} \label{lem:mod-layers}
%     Fix $t\in [m]$ which is a modified layer. There exists a constant $K(\epsilon)$ and a list of distributions $\cD_1\ldots \cD_{K(\eps)}$ over $[n]^2$ such that for every $\widehat{q_1},\widehat{q_2} \in \{0\ldots M\}$ with $t=\lfloor \log(\widehat{q_2}-\widehat{q_1}) \rfloor-1$, there exists $i$ such that
%     \[
%         \BigV \cD(\widehat{q_1},\widehat{q_2}), \cD_i \BigV_\TV \leq \eps^{9}.
%     \]
% \end{lemma}

We'll restate the lemma as follows.

\begin{lemma} \label{lem:nearby-crit}
    Fix $t\in [m]$ which is a modified layer. Then for every $\widehat{q_1},\widehat{q_2} \in \{0\ldots M\}$ and $\widehat{q_1^*},\widehat{q_2^*}$ satisfying the following:
    \begin{itemize}
        \item That $t=\lfloor \log(\widehat{q_2}-\widehat{q_1}) \rfloor-1$ and $t=\lfloor \log(\widehat{q_2^*}-\widehat{q_1^*}) \rfloor-1$.
        \item That $1-\eps^{200}<q_1/q_1^*<1+\eps^{200}$ and $1-\eps^{200}<(q_2-q_1)/(q_2^*-q_1^*)<1+\eps^{200}$.
    \end{itemize}
    It holds that TV distance between $\cD(\widehat{q_1},\widehat{q_2})$ and $\cD(\widehat{q_1^*},\widehat{q_2^*})$ is at most $\eps^{11}$.
\end{lemma}

\begin{proof}

\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:mod-layers}]
    trivial from Lemma~\ref{lem:nearby-crit}.
\end{proof}

\subsubsection{Proof of Lemma~\ref{lem:nonmod-layers}}

Before we proceed, we'll additionally need the following lemma, which happens to be a simple corollary of Lemma~\ref{lem:mod-layers}.

\begin{lemma}
    There exists a constant $K(\epsilon)$ and a list of distributions $\cD_1\ldots \cD_{K(\eps)}$ over $[n]$ such that for every $\widehat{q}$, there exists $i$ such that $\V \cD(\widehat{q}), \cD_i\V_\TV \leq \eps^{10}$.
\end{lemma}

\begin{proof}
    Take $\widehat{q_1}=0$ and $\widehat{q_2}=\widehat{q}$ in Lemma~\ref{lem:mod-layers}.
\end{proof}

% \begin{lemma} \label{lem:nonmod-layers}
%     Fix $t\in [m]$ which is not a modified layer. Then for every $\widehat{q_1},\widehat{q_2} \in \{0\ldots M\}$ with $t=\lfloor \log(\widehat{q_2}-\widehat{q_1}) \rfloor-1$, the following holds for at least $1-\eps^9$-fraction of the values of $\C(x)$. The distribution $\C(x)[\cD(\widehat{q_1},\widehat{q_2})]$ is within $\eps^{-9}$ of the distribution $\C(x)[\cD(\widehat{q_1})]^2$.
% \end{lemma}

\subsection{Concluding Lemma~\ref{lem:mod-layers} with an Info-Theoretic Argument} \label{sec:2query-info}

In this section, we conclude Theorem~\ref{thm:2query} using Lemma~\ref{lem:const-fns}. We restate the lemma below for convenience.

\constfns*

Throughout the rest of the proof, we'll let $K(\eps)$ be the constant from Lemma~\ref{lem:const-fns} and $\cF_1,\ldots , \cF_{K(\eps)}$ be the functions. Recall that the lemma says that performing any two query roughly takes the corresponding $\cF_i$ and samples the output of $\cF_i$ rather than performing the queries directly. The main notion we'll want to formalize to conlude Theorem~\ref{thm:2query} is that only being able to ask for the output of the $\cF_i$'s cannot tell us about all $N$ indices since there are only a constant number of $\cF_i$'s.


This implies the following lemma, which says that $x$ can be hashed down to a constant length corresponding to the outputs of $\cF_1(x),\ldots , \cF_{K(\eps)}(x)$ and any two-query outputs can be roughly determined from this hash.

\begin{lemma} \label{lem:hash}
    There exists a mapping $h : \{0,1\}^N \to \{0,1\}^{K(\eps)}$ so that for any two queries $\widehat{q_1},\widehat{q_2}$, there is a function $g_{\widehat{q_1},\widehat{q_2}} : \{0,1\}^{K(\eps)} \to \{0,1\}^2$ such that
    \[
        \BigV g_{\widehat{q_1},\widehat{q_2}}(h(x)), \C(x)[\cD(\widehat{q_1},\widehat{q_2})] \BigV_\TV \leq \eps^2.
    \]
\end{lemma}

\begin{proof}

\end{proof}

\begin{lemma} \label{lem:index-from-hash}
    Given any mapping $h : \{0,1\}^N \to \{0,1\}^{K(\eps)}$, there exists a constant $\kappa(\eps)$ so that for $N>\kappa(\eps)$, there exists $i\in [N]$ such that for uniformly random $x$, the index $x_i$ cannot be guessed correctly from $h(x)$ with probability more than $\frac12+\eps^2$.
\end{lemma}

\begin{proof}

\end{proof}

To conclude, we combine Lemma~\ref{lem:hash} and Lemma~\ref{lem:index-from-hash}. We let $h$ be the hash function chosen in Lemma~\ref{lem:hash}.

We assume for the sake of contradiction that $N>\kappa(\eps)$ as chosen in Lemma~\ref{lem:index-from-hash}. Then, there is some index that cannot be guessed correctly from $h(x)$ with probability more than $\frac12+\eps^2$ when $x$ is chosen uniformly at random. By Lemma~\ref{lem:hash} and using the definition of total variation distance, the output of the two queries can be simulated from $h(x)$ with probability at least $1-\eps^2$, so then the two queries cannot predict $x_i$ with probability more than $\frac12+\eps^2+\eps^2<\frac12+\eps$.

==> old-2query.tex <==
\subsection{Proof of Theorem~\ref{thm:2query}}

\begin{lemma} \label{lem:sameW}
    For any $k,\eps$ the following holds. Given any sequence $t_1<\ldots < t_{k/\eps^2}$ and any set of strings $S$, there exists $a$ with the following property. If we choose a string uniformly randomly from $S$, there is probability at least $1-\eps$ that $W_{t_{a+k}}(s)-W_{t_a}(s)<\eps$.
\end{lemma}

Throughout the rest, the set of strings will be $S=\{ECC(x)\}$ for all $x\in\{0,1\}^n$ where $n$ is a power of $2$. The deletion pattern will be: choose $\eps_1\in [\eps/4,\eps/2]$ and $\eps_2\in [\eps^2/4,\eps^2/2]$, and delete the first $\eps_1$ bits and then every remaining $1/\eps_2$th bit\footnote{could also delete them each with $\eps_2$ probability independently}. 

\begin{lemma} \label{lem:prod}
    For a given pair of queries $q, q+d$ to a string $s$ with the deletion pattern described above, the distribution of pairs it could possibly hit in the original query under the described deletion pattern can be modeled as follows. For $2^t\approx \frac{n}{d\eps^3}$, it is the product of pairs of intervals sized $n/2^t$, and the two entries are individually (but not jointly) distributed evenly over an interval of size $\eps n/4 n$.
    
\end{lemma}

\begin{proof}
    The two queries are
     $q(1+\eps_2)+n\eps_1$ and $(q+d)(1+\eps_2)+n\eps_1]$. This can be approximated as
    \[
        \Sigma_{a=0\ldots \frac{n}{\eps^2 4d}} \Sigma_{b=0\ldots 1/\eps^3} \left[q+\eps n/4+ a\eps^3 d,q+\eps n/4 + (a+1)\eps^3 d\right]
    \]
    \[
        \times\left[q+\eps n/4+ a\eps^3 d+d+\eps/4 d + b\eps^3 d,q+\eps n/4+ a\eps^3 d+d+\eps/4 d + (b+1)\eps^3 d\right]
    \]
    which basically satisfies the assertion in the lemma, if you shift intervals a bit to be in the powers of 2 division.
\end{proof}

We now return to the proof of the original problem.

\begin{proof}

Assume there are $1/\eps^{10}$ indices. Now, for every index $i$, take a good query $(q_i,q_i+d_i)$: that is one such that in expectation, averaging over all strings, making that query gives $>\frac12+\eps$ chance of success. Consider values of $i$ where $q_i$ is approximately the same: that is within distance $\eps^3 n$. Then, take $1/\eps^6$ of these $i$ values such that the values $d_i$ are mutually all at least a factor of 2 apart. If this isn't the case, many of them are within a factor of 2, and then the existing paper deals with this case (info theory argument). Let $2^{t_i}\approx n/d_i$, and relabeling the indices we have $t_1<\ldots<t_{1/\eps^6}$ Then we have a sequence for Lemma~\ref{lem:sameW}. WLOG, $t_1\ldots t_{1/\eps^3}$ all have the same value of $W_t(s)$ for most strings $s$.

Now we just need to put the elements together. The range of indices of the original string $s$ we care about is $[q+\eps n/4,q+\eps n/2]$. This corresponds to some number of chunks with $d=2^{t_1}$ ($t_1$ can be chosen large enough so this basically approximates the whole interval). Evaluating $W_{t_i}$ on only these chunks still preserves the property that all the $W_{t_i}$ are basically the same\footnote{probably need to modify Lemma~\ref{lem:sameW} to also show this}. This actually implies that the distribution of 0's and 1's doesn't change as you make the chunk more fine-grained (as $t$ increases). This in turn implies that for a given $i>1/\eps$, the probability you output each pair $11, 10, 01, 00$ is fully determined by the distribution of 0's and 1's in the chunks corresponding to $t_1$, since this is the same as the chunks corresponding to $t_{i+\log{\eps}}$, which are what actually determines it. Setting any threshold for guessing 0/1 for the value of the index simply cannot work if they're all giving each of $11, 10, 01, 00$ with equal probability, since on a random string you're expected to have about half 0's half 1's.
    
\end{proof}
